Detection of Uniform and Non-Uniform Differential Item Functioning by Item Focussed Trees

Detection of differential item functioning by use of the logistic modelling approach has a long tradition. One big advantage of the approach is that it can be used to investigate non-uniform DIF as well as uniform DIF. The classical approach allows to detect DIF by distinguishing between multiple groups. We propose an alternative method that is a combination of recursive partitioning methods (or trees) and logistic regression methodology to detect uniform and non-uniform DIF in a nonparametric way. The output of the method are trees that visualize in a simple way the structure of DIF in an item showing which variables are interacting in which way when generating DIF. In addition we consider a logistic regression method in which DIF can by induced by a vector of covariates, which may include categorical but also continuous covariates. The methods are investigated in simulation studies and illustrated by two applications.

==> header.tex <==
%% neu 1.9.2011     Abstände zwischen den Einträgen des Literaturverzeichnisses variieren.



%% Schrift
%\usepackage{mathptmx}
%\usepackage[scaled=.90]{helvet}
%\usepackage{courier}



\usepackage{times}      % old but good
%\usepackage{lmodern} %Latex STandard Schrift


%% language, coding
\usepackage[german,english]{babel}
\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage[latin1]{inputenc}

\usepackage{afterpage}

\usepackage{multind}             %multiple Inidices



\usepackage{chicago_new}




\usepackage{amsfonts, amsmath, amssymb, amsthm}
\usepackage{calc}
\usepackage{curves,epic,eepic,latexsym,ifthen}
%new
\usepackage{curves,epic,eepic,amsmath,latexsym,amssymb,array,ifthen,dcolumn}
\usepackage{epsfig}

%new
\usepackage{graphicx}
\usepackage[only,tenrm,svtnrm,egtrm,frtnrm]{rawfonts}

%\usepackage{showkeys}   %Label-Name at margin

\usepackage{rotating}
\usepackage{bbm}

\usepackage{color}
\usepackage{verbatim}
\usepackage{float}
\usepackage{textcomp}
\usepackage[english]{varioref}
\usepackage[scanall]{psfrag}

%Schauberger
\usepackage{tikz}
\usepackage{tikz-qtree}
\usepackage{pgfkeys}

\listfiles

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{%
  longtable,
  array,
  booktabs,
  dcolumn,
  rotating,
  shortvrb,
  tabularx,
  units,
  multirow
}

%\usepackage{fltpoint}
%\usepackage{rccol}
%\rcDecimalSign{.}


%% booktabs
\setlength{\heavyrulewidth}{0.06em}    % for \toprule and \bottomrule (default 0.08em)
\setlength{\lightrulewidth}{0.04em}    % for \midrulelightrulewidth (default 0.05em)
    % cmidrulewidht = 0.03em (fr \cmidrule)


%% Tables specific letter type
\newenvironment{tabularsmall}
{
\footnotesize \sffamily
\tabular
}
{
\endtabular
\normalfont
}

%% Ausrichtung am Dezimalpunkt
\newcolumntype{d}[1]{D{.}{.}{#1}} %% d{Anz.Dezimalstellen}


\newcolumntype{.}[1]{D{.}{.}{#1}}  %% in count


%% zum leichteren Ausrichten von Tabellenspalten
\newcommand{\ph}[1]{\phantom{#1}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Pages, Margins
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[
DIVcalc,       % Textbereich (in log-Datei nachlesen)
%DIVclassic
%,headinclude    % dann ist Kopfzeile+Text 18,9cm hoch,
%,headexclude    % dann ist nur der Text 18.9cm hoch + Kopfzeile
%,footexclude    % footinclude
,1.0headlines   %default ist 1.25headlines
%,pagesize
]{typearea}

%\typearea{8}

%\areaset{11.7cm}{18.9cm}
\areaset{13.3cm}{21.0cm}
%kleinerer Abstand von Kopfzeile zu Text
%\setlength{\headheight}{0pt} %13.6pt    holt den Text etwas nï¿½er



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         fancy head and bottom
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{fancyhdr}

\pagestyle{fancy}
\lhead[\fancyplain{}{\textrm\thepage}]                            % even page
      {\fancyplain{}{\normalfont\footnotesize\scshape\rightmark}} % uneven page
\rhead[\fancyplain{}{\normalfont\footnotesize\scshape\leftmark}]
      {\fancyplain{}{\textrm\thepage}}
\chead{}

\renewcommand{\headrulewidth}{0.5pt} % Trennlinie
\setlength{\headsep}{10pt}           % kleinerer Abstand Text-Kopfzeile (default ist 25pt)

\lfoot{}
\cfoot{\fancyplain{\textrm\thepage}{}}
\rfoot{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  minipages with boxes
% use  \boxnew[Breite]{Inhalt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\boxtitle}[1]{\begin{center} \sffamily #1 \end{center}}
\newcommand{\boxitem}[1]{\textsf{\small #1}}

\newcommand{\boxnew}[2][0.8\textwidth]{               %0.8\textwidth als default
   \vspace{1.5ex}          %1ex bewirkt nichts, entspricht 100%
   \begin{center}
   \fbox{%
     \begin{minipage}{#1}   %\linewidth-4ex  ergibt textbreiten Kasten
       {#2}%
     \end{minipage}}%
   \end{center}
   \vspace{2ex}
}

\newcommand{\boxcaption}[1]{
\captionsetup{aboveskip=-1.6ex, belowskip=2ex}
\captionof{table}{#1}
\captionsetup{aboveskip=10pt, belowskip=0pt}
\vspace{1.5ex}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Index (neu 6.7.06 von J.Brandt)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sindex}[1]{\index{subjectindex}{#1}}
\newcommand{\aindex}[1]{\index{authorindex}{#1}}

% Zweispaltiger Index
\makeatletter
\renewcommand{\printindex}[2]{
   \@restonecoltrue\if@twocolumn\@restonecolfalse\fi
   \columnseprule \z@ \columnsep 35pt   %%obsolet, besser \setlength
   \newpage
   \@mkboth{\MakeUppercase{#2}}{\MakeUppercase{#2}}      %Fr Kopfzeile
%    \twocolumn[{\rm\huge\sffamily\mdseries #2 \vskip4ex}]      %%obsolet, wegen \rm
    \twocolumn[{\rm\huge\sffamily\mdseries #2 \vskip4ex}]
   \addcontentsline{toc}{chapter}{#2}                    %Eintrag ins Inhaltsverzeichnis
   \@input{#1.ind}
 }
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Examples including counter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcommand{\ecaption}[1]{\addcontentsline{loe}{example}{\protect\numberline{\theexample}#1}} %loe: listOfExamples
\newcommand{\l@example}{\@dottedtocline{1}{0em}{3.2em}}

\newcommand{\listofexamples}{
     \chapter*{List of Examples}                  %ï¿½berschrift der Beispielsliste
     \@mkboth{List of Examples}{List of Examples}         %header
%   \addcontentsline{toc}{section}{List of Examples}    %hier liegt das Problem mit den minitocs => statt chapter nun section und es funktioniert
\addcontentsline{toc}{chapter}{List of Examples}
%     \thispagestyle{empty}
     { \@starttoc{loe}}
}
\makeatother

\newcounter{example}[chapter]
\renewcommand{\theexample}{\thechapter.\arabic{example}}

\newenvironment{example}[1]
    {\refstepcounter{example}
     \ecaption{#1}
     \bigskip
     \noindent{\small \sffamily Example \theexample: #1}
     %\noindent{\small \scshape Example \normalfont \theexample: #1}
                    % Schrift der Beispielsberschrift
     \small         % Schrift des Textes (ohne ï¿½berschrift)
     \\}
    {\qed \bigskip}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Chapter headings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
%% aus book.cls kopiert und modifiziert
\renewcommand\chapter{\if@openright\cleardoublepage\else\clearpage\fi
                    \thispagestyle{plain}%
                    \global\@topnum\z@
                    \@afterindentfalse
                    \secdef\@chapter\@schapter}
\def\@chapter[#1]#2{\ifnum \c@secnumdepth >\m@ne
                       \if@mainmatter
                         \refstepcounter{chapter}%
                         \typeout{\@chapapp\space\thechapter.}%
                         \addcontentsline{toc}{chapter}%
                                   {\protect\numberline{\thechapter}#1}%
                       \else
                         \addcontentsline{toc}{chapter}{#1}%
                       \fi
                    \else
                      \addcontentsline{toc}{chapter}{#1}%
                    \fi
                    \chaptermark{#1}%
                    \addtocontents{lof}{\protect\addvspace{10\p@}}%
                    \addtocontents{lot}{\protect\addvspace{10\p@}}%
                    \if@twocolumn
                      \@topnewpage[\@makechapterhead{#2}]%
                    \else
                      \@makechapterhead{#2}%
                      \@afterheading
                    \fi}
\def\@makechapterhead#1{%
  \vspace*{50\p@}%
  {\parindent \z@ \raggedright \sffamily  %\normalfont default, jetzt \sffamily
    \ifnum \c@secnumdepth >\m@ne
      \if@mainmatter
        \huge \@chapapp\space \thechapter %\bfseries  %nur fï¿½r das Wort Chapter
        \par\nobreak
        \vskip 20\p@        %20
      \fi
    \fi
    \interlinepenalty\@M
%    \Huge  #1\par\nobreak  %\bfseries       %fï¿½r die eigentliche ï¿½berschrift
    \huge  #1\par\nobreak  %\bfseries
    \vskip 40\p@        %40
  }}
\def\@schapter#1{\if@twocolumn
                   \@topnewpage[\@makeschapterhead{#1}]%
                 \else
                   \@makeschapterhead{#1}%
                   \@afterheading
                 \fi}
\def\@makeschapterhead#1{           %verï¿½ndert die Schrift der ï¿½berschrift des Inhalts-, Beispiels- und Literaturverzeichnisses
  \vspace*{50\p@}%
  {\parindent \z@ \raggedright
    \sffamily                       %\normalfont alt
    \interlinepenalty\@M
%    \Huge   #1\par\nobreak          %\bfseries
    \huge   #1\par\nobreak
    \vskip 40\p@
  }}
%%

\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}% Abstand drï¿½ber
                                   {1.1ex \@plus.1ex}      % Abstand drunter
                                   {\sffamily\Large}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
                                     {1.0ex \@plus .1ex}%
                                     {\sffamily\large}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
                                     {0.5ex \@plus .1ex}%
                                     {\sffamily\normalsize}}
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                    {3.25ex \@plus1ex \@minus.2ex}%
                                    {1ex}%
                                    {\sffamily\normalsize}}
\makeatother

%default-Werte
% \newcommand\section{\@startsection {section}{1}{\z@}%
%                                    {-3.5ex \@plus -1ex \@minus -.2ex}%
%                                    {2.3ex \@plus.2ex}%
%                                    {\normalfont\Large\bfseries}}
% \newcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                      {-3.25ex\@plus -1ex \@minus -.2ex}%
%                                      {1.5ex \@plus .2ex}%
%                                      {\normalfont\large\bfseries}}
% \newcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-3.25ex\@plus -1ex \@minus -.2ex}%
%                                      {1.5ex \@plus .2ex}%
%                                      {\normalfont\normalsize\bfseries}}
% \newcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
%                                     {3.25ex \@plus1ex \@minus.2ex}%
%                                     {-1em}%
%                                     {\normalfont\normalsize\bfseries}}
% \newcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
%                                        {3.25ex \@plus1ex \@minus .2ex}%
%                                        {-1em}%
%                                       {\normalfont\normalsize\bfseries}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Im Anhang bekommen chapter, section und subsection wieder andere Bedeutung
% (noch nicht berarbeitet)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \makeatletter
%   \renewcommand*\l@chapter[2]{%
%     \ifnum \c@tocdepth >\m@ne
%       \addpenalty{-\@highpenalty}%
%       \vskip 1.0em \@plus\p@
%       \setlength\@tempdima{1.5em}%
%       \begingroup
%         \parindent \z@ \rightskip \@pnumwidth
%         \parfillskip -\@pnumwidth
%         \leavevmode \bfseries %\mdseries %\sffamily
%         \advance\leftskip\@tempdima
%         \hskip -\leftskip
%         #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
%         \penalty\@highpenalty
%       \endgroup
%     \fi}
% \renewcommand{\appendixname}{Appendix}
% \renewcommand{\appendix}{%
%   \setcounter{chapter}{0}
%   \renewcommand{\thechapter}{\Alph{chapter}}%
%   \renewcommand{\chapter}[1]{%
%     \cleardoublepage\thispagestyle{plain}%
%     \refstepcounter{chapter}%
%     \addcontentsline{toc}{chapter}%
%       {%\protect\sffamily%
%        \protect\numberline{\protect\bfseries\protect%   %%dazw.\bfseries
%        \protect\appendixname\protect\hspace{1ex}\thechapter:}\protect\hspace{9ex}\protect##1}%
%     \@mkboth{\MakeUppercase{\appendixname\ \thechapter:\ ##1}}%
%             {\MakeUppercase{\appendixname\ \thechapter:\ ##1}}%
%     {\flushleft\LARGE\mdseries\sffamily%
%      \appendixname\ \thechapter:\ \nohyphens##1\par}%
%   %\chaptermark{##1}\vspace{\baselineskip}
%   }
%   \renewcommand{\section}[1]{
%     \refstepcounter{section}%
%     \addcontentsline{toc}{section}%
%       {%\protect\sffamily%
%        \protect\numberline{\thesection}##1}%
%     {\noindent\large\mdseries\sffamily\thesection~##1\par}
% %    {\flushleft\large\mdseries\sffamily\thesection~##1\par} ohne Trennungen
%   }
%   \renewcommand{\subsection}[1]{
%     \refstepcounter{subsection}%
%     \addcontentsline{toc}{subsection}%
%       {%\protect\sffamily%
%        \protect\numberline{\thesubsection}##1}%
%     {\noindent\normalsize\mdseries\sffamily\thesubsection~##1\par}
% %    {\flushleft\normalsize\mdseries\sffamily\thesubsection~##1\par} ohne Trennungen
%   }
% }
%% \makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Captions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{caption}[2003/12/20]
\captionsetup{width=\linewidth-2cm,font=footnotesize,labelfont={sc}}
    %font: Einstellung fï¿½r die gesamte Unterschrift
    %labelfont: Einstellung fï¿½r den Bezeichner (``Table'')


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Literature  - neu 1.9.2011 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% aus book.cls %%

\makeatletter

\renewenvironment{thebibliography}[1]
     {\chapter*{\bibname}%
      \@mkboth{\MakeUppercase\bibname}{\MakeUppercase\bibname}%
      %     {\rm\Large\sffamily\mdseries \bibname\vskip2ex}     %ergänzt
    \addcontentsline{toc}{chapter}{\bibname}    %ergänzt
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}

\makeatother

\let\oldbibliography\thebibliography
\renewcommand{\thebibliography}[1]{%
\oldbibliography{#1}%
%\setlength{\itemsep}{0ex}           %% Abstand zwischen den Einträgen %%
\setlength{\itemsep}{-0.3ex} }




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         minitocs: kleine Inhaltsverzeichnisse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{minitoc}       % kleine Inhaltsverzeichnisse
\setlength{\fboxsep}{1em}  % \fboxsep4mm    %Vergleiche Einstellungen fï¿½r \boxnew
\setlength{\mtcindent}{4pt}
\renewcommand{\mtcfont}{\small\mdseries\sffamily}
\renewcommand{\mtcSfont}{\small\mdseries\sffamily}
\renewcommand{\mtcSSfont}{\small\mdseries\sffamily}

\newcommand{\makeminitoc}{%
\setcounter{minitocdepth}{3}    % Anzahl Gliederungsebenen
   \vspace{3mm}
   \hrule
   \bigskip
   \noindent


%   \fbox{%
   \begin{minipage}{\linewidth -5ex}
     \vspace*{-3ex}
     \nomtcrule
     \minitoc
\hrule
\bigskip
%     \vspace*{-5ex}%3
   \end{minipage}
%   }
\\[3mm]}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%          Applications   ** neu 21.10.09 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ZÃ¤hler fÃ¼r die Applications innerhalb der Umgebung
\newcounter{application}[chapter]
\renewcommand{\theapplication}{\thechapter.\arabic{application}}

%% Definition der Umgebung 'application'
\newenvironment{application}
    {\refstepcounter{application}
     \bigskip
     \noindent{\small \sffamily Application \theapplication:} % Ãberschrift
     \\
     \small         % Schrift des Textes (ohne Ueberschrift)
     }

    { \bigskip}

%% Fuer leichtere (a), (b), (c) AufzÃ¤hlungen
\usepackage{enumitem}

\newenvironment{abcitemize}
    {\begin{enumerate}[label=(\alph*)]}
    {\end{enumerate}}


% \newenvironment{anwendung}[1]
%     {\refstepcounter{application}
%      \bigskip
%      \noindent{\small \sffamily Application \theapplication:} % Ãberschrift
%      \small         % Schrift des Textes (ohne Ueberschrift)
%      \\
%      #1
%      \begin{enumerate}[label=(\alph*)]
%      }
%     { \end{enumerate} \bigskip}







% %% Variante 2 *****************************************************************

%
%
% \renewcommand{\labelenumi}{\small \textsf{Application \theenumi :}}
%
%
% \newenvironment{anwendungen}%[Ã]
% {\small \begin{enumerate}[leftmargin=*, style=nextline] }
% {\end{enumerate} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%          Exercises   ** neu 19.11.09 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ZÃ¤hler fÃ¼r die Exercieses
\newcounter{exercise}[chapter]
\renewcommand{\theexercise}{\thechapter.\arabic{exercise}}

%% Definition der Umgebung 'exercise'
\newenvironment{exercise}
    {\refstepcounter{exercise}
     \bigskip \small
     \noindent \theexercise
     }

    { \bigskip}

